Productivity Beliefs and Efficiency in Science

We develop a method to estimate producers' productivity beliefs when output quantities and input prices are unobservable, and we use it to evaluate the market for science. Our model of researchers' labor supply shows how their willingness to pay for inputs reveals their productivity beliefs. We estimate the model's parameters using data from a nationally representative survey of researchers and find the distribution of productivity to be very skewed. Our counterfactuals indicate that a more efficient allocation of the current budget could be worth billions of dollars. There are substantial gains from developing new ways of identifying talented scientists.

==> figtab/note_fig_alpha_cites.tex <==
Shows the distribution of researchers' TFP ($\alpha_i$) and their field-normalized citations, where both metrics have been rescaled so the mean equals 1; note the log scale. 90-10 percentile ratios are also shown.


==> figtab/note_fig_bardiff_actvopt.tex <==
Shows the distribution of the input wedge, which equals a researcher's actual input level minus their optimal input level; positive values indicate the researcher is over-resourced and negative values indicate the researcher is under-resourced relative to the optimum.


==> figtab/note_fig_binscat_alpha_otherWTP.tex <==
Shows the implied dollar value of productivity in terms of the median (Panel A) or mean (Panel B) of in-sample researchers' willingness to pay for a given productivity level, where productivity ($ x$ axis) is scaled so that the sample mean equals one. For example, Panel (A) indicates that the median amount that researchers would be willing to pay to have average productivity is approximately \$1,000 per year. Note, negative values imply that researchers must be paid to receive a given productivity level (because it is lower than their current productivity).


==> figtab/note_fig_dens_time.tex <==
Shows the distribution of researchers' hours per week spent on four categories of work tasks.


==> figtab/note_fig_dens_totalbudget.tex <==
Shows the distribution of researchers' total expected annual research budget (including guaranteed funds plus fundraising expectations) split by the researchers' major field of study; note the log scale.


==> figtab/note_fig_dmalpha_bymajor.tex <==
TEST.


==> figtab/note_fig_fielddens_OA.tex <==
Shows the distribution of researchers' hours per week spent on teaching, administration, clinical, or other duties by major field.


==> figtab/note_fig_hist_actvopt.tex <==
Shows the distribution of actual and optimal input levels. Panels (a--b) show the distribution of the inputs assumed to be directly under the planners' control. Panels (c--d) show the distribution of inputs after researchers' choose their time allocations in response to the planner.


==> figtab/note_fig_metasci_openalex.tex <==
Shows the share of all research publications related to meta-science within each publication database.


==> figtab/note_fig_modelfit_answprederro_0.tex <==
Panel (A) shows the distribution of researchers' responses to the four experiments (i.e., their stated annual salary at indifference) alongside the distribution of the model's predictions and absolute errors. Panel (B) reports summary statistics for the distribution of the absolute errors for each of the four experiments where the model's errors are expressed in percentage points of the actual responses.


==> figtab/note_fig_modelfit_answprederro_1.tex <==
Panel (A) shows the distribution of researchers' responses to the four experiments (i.e., their stated annual salary at indifference) alongside the distribution of the model's predictions and absolute errors. Panel (B) reports summary statistics for the distribution of the absolute errors for each of the four experiments where the model's errors are expressed in percentage points of the actual responses.


==> figtab/note_fig_nonresponse_dim.tex <==
Panel (a) shows the distribution of publication and grant outcomes split by whether the researcher was emailed (i.e., the full sample) versus those who completed the survey; note the log $ x$ axes. Panel (b) reports estimates from a regression of each measure on a binary indicator for whether the researcher completed the survey; \emph{\% diff.} reports this difference in percentage terms. Robust standard errors reported; $^{*} p<0.10, ^{**} p<0.05, ^{***} p<0.01$.


==> figtab/note_fig_nonresponse_herd.tex <==
Panel (a) shows the distribution of institutional funding measures split by whether the researcher was emailed (i.e., the full sample) versus those who completed the survey. Panel (b) reports estimates from a regression of each measure on a binary indicator for whether the researcher completed the survey; \emph{\% diff.} reports this difference in percentage terms. Robust standard errors reported; $^{*} p<0.10, ^{**} p<0.05, ^{***} p<0.01$.


==> figtab/note_fig_topa_powerlaw01.tex <==
Shows the log rank of researchers' TFP ($\alpha_i$, where the sample mean is normalized to 1) versus the log of the TFP for the top 1\% of researchers. The power law exponent reported is based on the linear regression of log rank on log TFP (see the dashed line) following \cite{gabaix2009power}.


==> figtab/note_fig_topa_powerlaw05.tex <==
Shows the log rank of researchers' TFP ($\alpha_i$, where the sample mean is normalized to 1) versus the log of the TFP for the top 1\% of researchers. The power law exponent reported is based on the linear regression of log rank on log TFP (see the dashed line) following \cite{gabaix2009power}.


==> figtab/note_fig_topa_powerlaw10.tex <==
Shows the log rank of researchers' TFP ($\alpha_i$, where the sample mean is normalized to 1) versus the log of the TFP for the top 10\% of researchers. The power law exponent reported is based on the linear regression of log rank on log TFP (see the dashed line) following \cite{gabaix2009power}.


==> figtab/note_fig_topa_powerlaw20.tex <==
Shows the log rank of researchers' TFP ($\alpha_i$, where the sample mean is normalized to 1) versus the log of the TFP for the top 20\% of researchers. The power law exponent reported is based on the linear regression of log rank on log TFP (see the dashed line) following \cite{gabaix2009power}.


==> figtab/note_tab_counterfac_summaries_alt.tex <==
Reports summary statistics for inputs and outcomes under actual allocations (Col. 1) and the utility-maximizing allocation (Cols. 2--5). Column (2) reports the main results from our preferred specification. Columns (3--5) report results under alternative specifications of the model and its estimation. \emph{Absolute input cap} refers to the scenario where researchers' behavioral responses are limited with a global absolute maximum (as opposed to a relative maximum in the preferred scenario). \emph{Homogeneous param.} refers to the scenario where all non-production-function parameters are homogeneous. \emph{Across field $ B$} allows for the reallocation of inputs across the five major fields of study (which is not allowed in the preferred scenario).


==> figtab/note_tab_hetindex_ttest.tex <==
Reports a t-test of the difference in means between the two predicted clusters following the $ k$-means cluster estimation with $ k$=2; $^{*} p<0.10, ^{**} p<0.05, ^{***} p<0.01$.


==> figtab/note_tab_reg_alpha_triplet.tex <==
TEST.


==> figtab/note_tab_reg_wedger2.tex <==
Reports $ R^2$ statistics from regressions of the input wedge (i.e., actual minus optimal input levels) on different subsets of covariates $ \mathbf{X}$ used to construct the type index; \emph{position} covariates include researchers' rank and tenure status; \emph{output} covariates include researchers' Likert-scale based reporting of the intended outputs (e.g., publications, books) and audiences (e.g., peers, policymakers) of their research; \emph{socio-demog.} covariates include measures of household structure, race/ethnicity, nationality, and gender.


==> figtab/note_tab_sumstat_minorfield.tex <==
Reports the share of 4,003 researcher-level observations in each minor field.


==> figtab/note_tab_sumstat_othervar.tex <==
Reports summary statistics for 4,003 researcher-level observations. \emph{From HERD} indicates variables from \cite{nsf2023herd}. \emph{From Dimensions} indicates variables from the \cite{dimension2018data} dataset. \emph{N.R.} stands for Not Reported.


==> figtab/note_tab_sumstat_othervar2.tex <==
Reports summary statistics for 4,003 researcher-level observations. \emph{N.R.} stands for Not Reported.


==> figtab/note_tab_wedgereg_sociodemog.tex <==
Reports results from regressions of actual input levels on optimal input levels and a binary indicator for female gender. Research time is in units of hours per week, and research funding is in units of \$ per year. Robust standard errors reported; $^{*} p<0.10, ^{**} p<0.05, ^{***} p<0.01$.


==> figtab/note_tab_wedgereg_sociodemog_age.tex <==
Reports results from regressions of actual input levels on optimal input levels and researchers' age. Research time is in units of hours per week, and research funding is in units of \$ per year. Robust standard errors reported; $^{*} p<0.10, ^{**} p<0.05, ^{***} p<0.01$.


==> figtab/note_tab_wtp_tests.tex <==
TEST.


==> figtab/stub_maincounterfact_dU.tex <==
5

==> figtab/stub_maincounterfact_dY.tex <==
160

==> figtab/stub_researcherlevel_vardecomp_BR.tex <==
28


==> figtab/stub_researcherlevel_vardecomp_fieldspecific_a.tex <==
42--66


==> figtab/stub_researcherlevel_vardecomp_g.tex <==
26


==> figtab/tab_par_estimates.tex <==

	\begin{tabular}{llll}
		\hline \hline
		& Parameter & Symbol & Value \\
		\hline
		Income & Curvature  & $\sigma$ & 0.4598 \\
		Research Output & Level & $\kappa$ & 1.38 $\times$ $10^{-5}$ \\
		& Curvature & $\eta$ & 0.234 \\
		Labor & Level & $\psi$ & 0.001 \\
		& General Curvature & $1+\zeta$ & 1 \\
            & Duties Curvature & $\xi$ & 1.490 \\
		\hline
            \hline
	\end{tabular}



==> paper_Zfigtab.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Tables \& Figures}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{10em}
\begin{table}[hp]\centering \small
\caption{Summary Statistics---Salary, Funding, Time, and Fields}\label{tab_sumstat_modelvar}
\-\\
\input{figtab/tab_sumstat_modelvar.tex}
\-\\
\note{\emph{Note}: \input{figtab/note_tab_sumstat_modelvar.tex}} 
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage\begin{table}[p]\centering \small
\caption{Summary Statistics---Subjective Output}\label{tab_sumstat_qualoutput}
\-\\
\input{figtab/tab_sumstat_qualoutput.tex}
\-\\
\note{\emph{Note}: \input{figtab/note_tab_sumstat_qualoutput.tex}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage\begin{figure}[p] \centering
\caption{Willingness to Pay Experiment Responses}\label{fig_hist_wtp}
\subfloat[WTP for +\$1 Research Funding]
{
\label{fig_hist_wtp_dols}
\includegraphics[width=0.495\textwidth, trim=0mm 20mm 0mm 5mm, clip]{figtab/fig_hist_wtp_dols.png}
} 
\subfloat[WTP for --1 hr. Administrative Duties]
{
\label{fig_hist_wtp_hr}
\includegraphics[width=0.495\textwidth, trim=0mm 20mm 0mm 5mm, clip]{figtab/fig_hist_wtp_hr.png}
} \\
\note{\emph{Note}: \input{figtab/note_fig_hist_wtp.tex}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage\begin{figure}[p] \centering
\caption{Utility Function Visualization}\label{fig_util}
\subfloat[Salary, $M$]
{
\label{fig_util_M}
\includegraphics[width=0.475\textwidth, trim=0mm 10mm 0mm 5mm, clip]{figtab/fig_util_M.png}
} 
\subfloat[Administrative Duties, $D$]
{
\label{fig_util_A}
\includegraphics[width=0.475\textwidth, trim=0mm 10mm 0mm 5mm, clip]{figtab/fig_util_A.png}
}
\\ \-\\ \-\\
\subfloat[Guaranteed Research Budget, $G$]
{
\label{fig_util_G}
\includegraphics[width=0.475\textwidth, trim=0mm 10mm 0mm 5mm, clip]{figtab/fig_util_G.png}
}
\subfloat[Research Output, $Y$]
{
\label{fig_util_Y}
\includegraphics[width=0.475\textwidth, trim=0mm 10mm 0mm 5mm, clip]{figtab/fig_util_Y.png}
}
\-\\
\note{\emph{Note}: \input{figtab/note_fig_util.tex}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage\begin{figure}[p] \centering
\caption{Production Function Parameters}\label{fig_hist_pfunc}
\subfloat[Funding intensity, $\gamma$]
{
\label{fig_hist_pfunc_gamma}
\includegraphics[width=0.495\textwidth, trim=0mm 20mm 0mm 5mm, clip]{figtab/fig_hist_pfunc_gamma.png}
} 
\subfloat[Scaled TFP, $\alpha$]
{
\label{fig_hist_pfunc_alpha}
\includegraphics[width=0.495\textwidth, trim=0mm 20mm 0mm 5mm, clip]{figtab/fig_hist_pfunc_alpha.png}
} \\
\note{\emph{Note}: \input{figtab/note_fig_hist_pfunc.tex}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage\begin{figure}[p] \centering
\caption{TFP Distributions}\label{fig_alpha_distcompare}
\includegraphics[height=0.5\textwidth, trim=0mm 10mm 0mm 5mm, clip]{figtab/fig_alpha_distcompare.png}
\-\\
\note{\emph{Note}: \input{figtab/note_fig_alpha_distcompare.tex}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage\begin{figure}[p] \centering
\caption{Power Laws in the TFP Tail}\label{fig_topa_powerlaw}
\subfloat[Top 20\% Researchers]
{
\label{fig_topa_powerlaw20}
\includegraphics[width=0.495\textwidth, trim=5mm 20mm 0mm 5mm, clip]{figtab/fig_topa_powerlaw20.png}
} 
\subfloat[Top 1\% Researchers]
{
\label{fig_topa_powerlaw01}
\includegraphics[width=0.495\textwidth, trim=5mm 20mm 0mm 5mm, clip]{figtab/fig_topa_powerlaw01.png}
} \\
\note{\emph{Note}: \input{figtab/note_fig_topa_powerlaw.tex}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage\begin{table}[p]\centering \small
\caption{Outcomes given Actual and Optimized Allocations}\label{tab_maincounterfac_summaries}
\-\\
\input{figtab/tab_maincounterfac_summaries.tex}
\-\\
\note{\emph{Note}: \input{figtab/note_tab_maincounterfac_summaries.tex}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage\begin{figure}[p] \centering
\caption{Actual and Optimal Input Level Correlations}\label{fig_binscat_actvopt}
\subfloat[Research Time]
{
\label{fig_binscat_actvopt_C_Ri}
\includegraphics[width=0.475\textwidth, trim=0mm 10mm 0mm 5mm, clip]{figtab/fig_binscat_actvopt_C_Ri.png}
} 
\subfloat[Total Research Funding]
{
\label{fig_binscat_actvopt_C_Bi}
\includegraphics[width=0.475\textwidth, trim=0mm 10mm 0mm 5mm, clip]{figtab/fig_binscat_actvopt_C_Bi.png}
}
\-\\
\note{\emph{Note}: \input{figtab/note_fig_binscat_actvopt.tex}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage\begin{table}[p]\centering \small
\caption{Growth in Funding with Actual Allocations Needed to Produce the Same Output \\ as Optimized Allocation of Actual Funding}\label{tab_alternatives}
\-\\
\input{figtab/tab_alternatives.tex}
\-\\
\note{\emph{Note}: \input{figtab/note_tab_alternatives.tex}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage\begin{figure}[p] \centering
\caption{Across Field Output Comparisons}\label{fig_output_decomp}
\includegraphics[width=\textwidth, trim=0mm 10mm 0mm 5mm, clip]{figtab/fig_output_decomp.png}
\-\\
\note{\emph{Note}: \input{figtab/note_fig_output_decomp.tex}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
